Towards an Holistic Definition of Requirements Debt

When not appropriately managed, technical debt is considered to have negative effects on the long term success of a software project. However, how the debt metaphor applies to requirements engineering in general, and to requirements engineering activities in particular, is not well understood. Grounded in the existing literature, we present a holistic definition of requirements debt which include debt incurred during the identification, formalization, and implementation of requirements. We outline future assessment to validate and further refine our proposed definition. This conceptualization is the first step towards a requirements debt monitoring framework to support stakeholders decisions, such as when to incur and eventually pay back requirements debt, and at what costs

==> Sections/Approach.tex <==
\section{Roadmap}
\label{Approach}
\todo[inline,color=green,author=Davide]{Non mi sembra necessaria questa sezione. Rimuovi o includi nella intro.}
Overall, the research objectives and outcomes of this proposal are:
\begin{itemize}
 \item \textbf{Requirement Debt (ReD) definition}. We aim at extend the current ReD definition~\cite{Ernst2012} including upstream activities.
 \item \textbf{Requirement Debt detection}. 
 \item \textbf{Requirement Debt quantification}. 
 \item \textbf{Requirement Debt pay back}. 
 \item \textbf{Definition of a framework}. We aim at defining framework that can help stakeholders to make decisions regarding when to incur debt, at what costs, when to pay it back, and how to monitor it. 
\end{itemize}






==> Sections/Discussion.tex <==
\section{Discussion}
\label{Discussion}

==> Sections/Results.tex <==
\section{Result}
\label{Result}
